The importance of fillers for text representations of speech transcripts

While being an essential component of spoken language, fillers (e.g."um" or "uh") often remain overlooked in Spoken Language Understanding (SLU) tasks. We explore the possibility of representing them with deep contextualised embeddings, showing improvements on modelling spoken language and two downstream tasks - predicting a speaker's stance and expressed confidence.

==> background.tex <==
\label{background}
Studies on fillers often focus on their comprehension by the listener \cite{corley2008hesitation}, as their meaning is highly contextual, and dependent on the listener's interpretation \cite{Clark2002_using}. A speaker therefore encodes meaning into their speech, while the listener decodes (perceives) this meaning \cite{grice1975logic}. \citet{Brennan1995_feeling} observed that fillers and prosodic cues contribute to the listener's perception of the speaker's expressed confidence/ commitment to their utterance, which they refer to as the \textit{Feeling of Another's Knowing (FOAK)}, also observed by \cite{wollermann2013disfluencies}.
Besides their link to a speaker's metacognitive state, fillers have been studied for their role in discourse. Fillers frequently occur at the start of the discourse boundaries \cite{swerts1998filled,Shriberg2001_errrr,swerts1994prosody,Yoshida2010_disfluency}, which could indicate production difficulties of the speaker, while signalling to the listener to anticipate new/upcoming information. Few studies focus solely on the textual representation of fillers in a machine learning task (aside from disfluency detection). Using n-gram representations, fillers have been successful in \textit{stance} prediction \cite{le2017and}, and with disfluencies, \textit{turn-taking} prediction \cite{Saini2017_disfluency}, using one-hot vector representations to indicate their position in the utterance. \\ \indent
For our experiments, we use bidirectional encoder representations from transformers (BERT) \citet{devlin2018bert} because it has acheived SOTA performance on several NLP benchmarks, and to leverage contextualized word embeddings, which we believe is crucial for representing fillers. However, these embeddings are trained on written text (Wikipedia, BooksCorpus \cite{book}, Word Benchmark \cite{word_bench}). Earlier language representation models such as Word2Vec \cite{word2vec} perform poorly on tasks requiring context, such as word sense disambiguation. Despite being trained on textual data, research found that they did include word vectors for fillers, but could not correctly capture their contextual meanings \cite{valentin2017}. To our knowledge, no study has been conducted on the modelling of fillers to obtain a meaningful representation for spoken language modelling. 

%and Glove models \cite{pennington2014glove}

%(stance here referring to the subjective spoken attitudes towards something \cite{haddington2004stance})

%Their count is often taken as a feature in personality computing tasks \cite{park2014computational,vinciarelli2014survey}.

%Spoken language understanding have 1. ASR+NLU (Dilek paper, Ginzburg), with post processing, we have sentence boundary detection, disfluency removal etc? or end to end SLU (Micro Ravelli), found to be useful for low to high tasks. 
%FIND CITATION for this, there can be seperate pipelines for paralinguistic features (interspeech 2013) and lexical content, but not one that directly 
%spoken language transcripts?.
%SOmething about duplex?






==> notes.tex <==
TODO
- Still having difficulties with the track, asked a friend for feedback.
- Final editing, making sure terminology is consistent etc
- Supplementary stuff, re-write the stuff in RQ4 and add that table.
- Ask Chloe about conclusion and abstract
- Make (force) Pierre help comment some code after the paper
- CAN SAVE SPACE BY ABBREVIATING STUFF, esp spoken language modelling  

An abstract summarizes, usually in one paragraph of 300 words or less, the major aspects of the entire paper in a prescribed sequence that includes: 1) the overall purpose of the study and the research problem(s) you investigated; 2) the basic design of the study; 3) major findings or trends found as a result of your analysis; and, 4) a brief summary of your interpretations and conclusions.



\begin{algorithm}
\caption{Train LM}
\begin{algorithmic}
\REQUIRE Set. Proc. $S_{i}$, Token. Strat. $T_{i}$, Pretrained BERT $\mathcal{M}$.
\STATE $(\mathcal{D}_{train}, \mathcal{D}_{dev}, \mathcal{D}_{test}) \leftarrow$ (train, dev, test set) according to $S_{i}$
\IF{Do Finetuning}
\STATE $\mathcal{M} \leftarrow \mathcal{M}(\mathcal{D}_{train})$ using $(MLM,T_{i})$.
\ELSE
\STATE $\mathcal{M} \leftarrow \mathcal{M}$
\ENDIF

\STATE Evaluate: $Perplexity \leftarrow  \mathcal{M}$ on $\mathcal{D}_{test}$
\RETURN $(\mathcal{M},Perplexity)$ %
\end{algorithmic}
\label{algorithm:lm_training}
\end{algorithm}

\begin{algorithm}
\caption{Confidence prediction}
\begin{algorithmic}
\REQUIRE Set. Proc. $S_{i}$, Token. Strat. $T_{i}$, LM $\mathcal{M}$.
\STATE $(\mathcal{D}^{labelled}_{train}, \mathcal{D}^{labelled}_{dev}, \mathcal{D}^{labelled}_{test}) \leftarrow$ (train, dev, test set) according to $S_{i}$
\STATE $CONF_p \leftarrow \mathcal{M} + MLP $ 
\STATE $CONF_p \leftarrow CONF_p(\mathcal{D}^{labelled}_{train})$ using $(MSE,T_{i})$.

\STATE Evaluate: $MSE \leftarrow  CONF_p$ on $\mathcal{D}_{test}$
\RETURN $(CONF_p,MSE)$
\end{algorithmic}
\label{algorithm:conf_pred}
\end{algorithm}



\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
\caption{Confidence prediction}  %\textbf{**CC: standardize the notation with Algo 1 + we can not see here the fine-tuning steps}} 
\label{alg2} 
\begin{algorithmic}[1]
\REQUIRE Set. Proc. $\mathcal{P}_{Si}$, Token. Rep. $\mathcal{T}_i$, LM $\mathcal{LM}$ from \ref{alg1}.
\STATE $(\mathcal{D}^{labelled}_{train}, \mathcal{D}^{labelled}_{dev}, \mathcal{D}^{labelled}_{test}) \leftarrow$ (train, dev, test set) according to  ($\mathcal{P}_{Si}$,$\mathcal{T}_i$)
\STATE $CONF_p \leftarrow \mathcal{LM} + MLP $ 
\STATE $CONF_p \leftarrow CONF_p(\mathcal{D}^{labelled}_{train})$ using $(MSE)$.

\STATE Evaluate: $MSE \leftarrow  CONF_p$ on $\mathcal{D}_{test}$
\RETURN $(CONF_p,MSE)$
\end{algorithmic}
\end{algorithm}
\end{minipage}

\begin{figure*}
 \hline
\begin{minipage}{0.3\textwidth}
\begin{table}[H]
    \centering
\begin{tabular}{c|ccc} \hline
   Fine. &Setting & Token. & Ppl \\ \hline
    \vspace{0.05pt}
 \multirow{2}{*}{\rotatebox[origin=c]{90}{ w/o}}    & $\mathcal{P}_{S1}$/$\mathcal{P}_{S2}$& $\mathcal{T}_1$  & 22 \\
   & $\mathcal{P}_{S3}$& $\mathcal{T}_1$  & 20\vspace{0.05pt} \\ \hline
    \multirow{3}{*}{\rotatebox[origin=c]{90}{ w}}  &$ \mathcal{P}_{S1} $& $\mathcal{T}_1$  & 5.5 \\
    & $ \mathcal{P}_{S2}$& $\mathcal{T}_1$  & 5.6 \\
       & $\mathcal{P}_{S3}$& $\mathcal{T}_1$ & 4.6  \\
\end{tabular}
\caption{LM task.} % \textbf{**CC : change the notations of S+ standardize the number of significative numbers for perplexity (for example 2) : 22 20 5.5 5.6 4.6}
\label{table:SLM}
\end{table}

\end{minipage}
\hspace{15pt}
\begin{minipage}{0.3\textwidth}
\begin{table}[H]
    \centering
\begin{tabular}{ccc} \hline
  Setting & Token. & Ppl \\ \hline


    
        $\mathcal{P}_{S3}$& $\mathcal{T}_1$ & 4.6  \\
       
       $\mathcal{P}_{S3}$& $\mathcal{T}_2$  & 4.7 \\
     $ \mathcal{P}_{S3}$& $\mathcal{T}_3$   & 4.7 \\
     \vspace{10pt}
\end{tabular}

\caption{Best  $\mathcal{T}_i$}
\label{table:best_toke}
\end{table}

\end{minipage}
\begin{minipage}{0.3\textwidth}
\begin{table}[H]
    \centering
\begin{tabular}{c|cc} \hline
  BERT  & Model & MSE \\ \hline
 \multirow{2}{*}{w/o fine}   
   & $ \mathcal{P}_{S1} $ & 1.47 \\
    & $ \mathcal{P}_{S2} $ & 1.45 \\
     &  $\mathcal{P}_{S3}$  & \textbf{1.30} \\ \hline
    \multirow{2}{*}{w fine.}   
     
     &  $\mathcal{P}_{S1}$    & 1.32 \\
     &   $\mathcal{P}_{S2}$   & 1.31 \\
      &  $\mathcal{P}_{S3}$   & \textbf{1.24} \\
\end{tabular}
\caption{Confidence prediction. \textbf{**CC: change first column so that it is the same of TAble 2}}
\label{table:FOK_pred}
\end{table}

\end{minipage}
%\caption*{\textit{Fine} stands for fine-tuning. The model have been selected by the minimum of the training loss on the dev.}
\end{figure*}
